Simultaneous Topology Estimation and Synchronization of Dynamical Networks with Time-varying Topology

We propose an adaptive control strategy for the simultaneous estimation of topology and synchronization in complex dynamical networks with unknown, time-varying topology. Our approach transforms the problem of time-varying topology estimation into a problem of estimating the time-varying weights of a complete graph, utilizing an edge-agreement framework. We introduce two auxiliary networks: one that satisfies the persistent excitation condition to facilitate topology estimation, while the other, a uniform-$\delta$ persistently exciting network, ensures the boundedness of both weight estimation and synchronization errors, assuming bounded time-varying weights and their derivatives. A relevant numerical example shows the efficiency of our methods.

==> cdc_24_1/header.tex <==
%----------------------------------------------------------%
%-----------------------  Header file  --------------------%
%----------------------------------------------------------%

%------from IEEE template--v
	\usepackage{generic}
	\usepackage{cite}
	\usepackage{amsmath,amssymb,amsfonts}  % same as we use
	%\usepackage{algorithmic}
	\usepackage{anyfontsize}
	%\usepackage{graphicx,wrapfig}
	%\usepackage{textcomp}
	\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
			T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%	\markboth{Submitted to XXXX, \today}{Submitted to XXXX, \today}
	\markboth{\journalname, VOL. XX, NO. XX, XXXX 2023}
	{Restrepo \MakeLowercase{\textit{et al.}}: Simultaneous Topology Identification and Synchronization of Directed Dynamical Networks}
%------from IEEE template--^


% \IEEEoverridecommandlockouts
% \overrideIEEEmargins %With this it does not compile on the x270


%---layout stuff---v
	\parskip = 1pt 
	\allowdisplaybreaks
	\listfiles
%---layout stuff---^


%---- These lines are needed to activate hyperlinks, BEFORE \usepackage{hyperref} !!
% otherwise they do not work with ieeeconf.cls
	\makeatletter
	\let\NAT@parse\undefined
	\makeatother
	\usepackage[pdftex, pdfborderstyle={/S/U/W 0}]{hyperref}


%---packages for graphics & figures ----v
	\usepackage{graphicx,graphics,epsfig,color,wrapfig}
	\usepackage{float,subcaption}
	\usepackage{pgf,tikz,tikz-3dplot}
	\usepackage{tikzit}
	\usetikzlibrary{arrows,arrows.meta}
	\usetikzlibrary{positioning}
	\usepackage{pgfplots} 
	\usetikzlibrary{external}
	\tikzexternalize[prefix=Figures/]
	\newcommand{\inputtikz}[1]{%
		\tikzsetnextfilename{#1}%
		\input{#1}%
	}
%---packages for graphics & figures ----^


%--------other packages---------v
	\usepackage{threeparttable}
%	\usepackage[keeplastbox]{flushend}
%--------other packages---------^


%--- environments ---v
	\newtheorem{exe}{Example}
	\newtheorem{fact}{Fact}
	\newtheorem{rem}{Remark}
	\newtheorem{thm}{Theorem}
	\newtheorem{lem}{Lemma}
	\newtheorem{prop}{Proposition}
	\newtheorem{corol}{Corollary}
	\newtheorem{claim}{Claim}
	\newtheorem{defin}{Definition}
	\newtheorem{assump}{Assumption}
	
	% \newenvironment{proof}{{\it Proof. }}{\hfill $\blacksquare$}
	\newenvironment{example}{\ignorespaces\begin{exe}\rm }{\hfill $\square$ \end{exe}}
	\newenvironment{proposition}{\begin{prop}}{\hfill $\square$ \end{prop}}
	\newenvironment{corollary}{\begin{corol}}{\hfill $\square$ \end{corol}}
	\newenvironment{remark}{\begin{rem}}{\hfill $\bullet$ \end{rem}}
	\newenvironment{theorem}{\begin{thm}}{\hfill $\square$ \end{thm}}
	\newenvironment{lemma}{\begin{lem}}{\hfill $\square$ \end{lem}}
	\newenvironment{definition}{\vskip 3pt \begin{defin}}{\vskip 3pt \end{defin}}
	\newenvironment{assumption}{\vskip 3pt\begin{assump}}{\end{assump}\vskip 3pt}
%--- environments ---^


%---- Drafts ----v
%-----all these are only for the draft version -----v

	\usepackage{lipsum} 
	\newif\ifitsdraft
	\def\itsdraft{\global\itsdrafttrue}
	\newif\ifitsSPL
	\def\itsSPL{\global\itsSPLtrue}
	\newif\ifwithlualatex
	\def\withlualatex{\global\withlualatextrue}
	
	%\withlualatex   % <---- uncomment this line to compile with lualatex and tikz figures
	%\itsSPL
	%\itsdraft % <---- Uncomment to work in draft version
	
	\def\toremove#1{#1}  %--- command to remove material, eventually.
	%\def\toremove#1{}

	%--- some colours ---v
		\definecolor{myred}{rgb}{0.86,0.1,0.16}\def\myred#1{{\textcolor{myred}{#1}}}
		\definecolor{gray}{rgb}{0.3,0.3,0.3}\def\gray#1{{\textcolor{gray}{#1}}}
		\definecolor{lightgray}{rgb}{0.6,0.6,0.6}\def\lightgray#1{{\textcolor{lightgray}{#1}}}
		\definecolor{gray}{rgb}{0.33,0.4,0.47}\def\gray#1{{\color{gray}#1}}
		\definecolor{steelblue}{rgb}{0,.42,.7}\def\steelblue#1{{\color{steelblue}#1}}
		\definecolor{britishgreen}{rgb}{0,0.26,0.15}\def\britishgreen#1{{\color{britishgreen}#1}}
		\definecolor{navyblue}{rgb}{0,0,.8}\def\navyblue#1{{\color{navyblue}#1}}
		\definecolor{olivegreen}{rgb}{0.14,0.29,0}\def\olivegreen#1{{\color{olivegreen}#1}}
		\definecolor{myred}{rgb}{0.86,0.1,0.16}\def\myred#1{{\color{myred}#1}}
		
		\newcommand\red[1]{{\color{myred}#1}}
		\newcommand\blue[1]{{\color{blue}#1}}
	%--- some colours ---^


	\ifitsdraft %--- the following work only in Draft mode:
	
	\usepackage{refcheck}  
	\usepackage{soul}\onecolumn
	\usepackage[colorinlistoftodos,prependcaption,textsize=footnotesize,textwidth=2in]{todonotes}
	
	\onecolumn
	\textwidth=4.7in\oddsidemargin=0.3in\evensidemargin=0in%

	\newcounter{er}    \newcounter{al}    \newcounter{is}       \newcounter{todo}

	\newcommand{\ER}[2]{\stepcounter{er}\renewcommand{\baselinestretch}{0.9}%
		\texthl{#1}\todo[linecolor=red,backgroundcolor=red!1,bordercolor=red]{\color{black}ER(\theer): #2}%
		\renewcommand{\baselinestretch}{1}
	}

	\newcommand{\replace}[2]{\gray{\st{#1}}\ \navyblue{#2}}
	\newcommand{\ERreplace}[3]{\ER{}{\color{black} #3}\replace{#1}{#2}}    
	\newcommand{\rmk}[2]{
		\begin{quote}
			\color{navyblue} {\bf #1:} #2 \color{black}
		\end{quote}
	}

	\newcommand{\marginER}[2][0]%
	{\stepcounter{er}
		\todo[linecolor=red,backgroundcolor=red!1,bordercolor=red,noline]{\color{black}ER(\theer): #2}}

	\newcommand\todoin[1]{\stepcounter{er}
		\todo[inline, caption={}, linecolor=red,backgroundcolor=red!1, bordercolor=red]%
		{\begin{minipage}{\textwidth-4pt}\color{black}ER(\theer): #1\end{minipage}}}

	\newcommand{\inlineER}[1]
	{\stepcounter{er}
		\todo[linecolor=red,backgroundcolor=red!1,bordercolor=red,inline]{
			%                   \begin{minipage}{\textwidth-4pt} \color{black}AL(\theal):#1 \end{minipage}}}
			\color{black}ER(\theer): #1}}

	\newcommand{\IS}[2][0]{\stepcounter{is}\marginpar{
			\mbox{}\ \\[#1pt]
			\fontencoding{OT1}\fontsize{9.5}{10pt}\selectfont{
				\begin{minipage}[t]{2in}
					\hspace{5mm}\begin{minipage}[t]{2in} \color{steelblue}{ IS(\theis): #2} \end{minipage}
			\end{minipage}}
	}}
	\newcommand{\AL}[2][0]{\stepcounter{al}\marginpar{
			\mbox{}\ \\[#1pt]
			\fontencoding{OT1}\fontsize{9.5}{10pt}\selectfont{
				\begin{minipage}[t]{2in}
					\hspace{5mm}\begin{minipage}[t]{2in}
						\color{olivegreen}{\sf AL(\theal): #2}
			\end{minipage}\end{minipage}}
	}}

	\newcommand{\draftfootnote}[1]{\footnote{\color{gray}{\hrule \ \\ DRAFT FOOTNOTE: #1}}}
	
	\newcommand{\expendable}[2]{\stepcounter{er}\renewcommand{\baselinestretch}{0.9}%
		{\color{lightgray}#1}\todo[linecolor=red,backgroundcolor=red!1,bordercolor=red]{\color{black}ER(\theer): #2}%
		\renewcommand{\baselinestretch}{1}
	}

	\else
		\ifitsSPL   \onecolumn \textwidth=6.7in\oddsidemargin=0in\evensidemargin=0in%
		\renewcommand{\baselinestretch}{1.1}
	  \fi
		\newcommand{\expendable}[2]{\color{lightgray}#1\color{black}} 
		\newcommand\todoin[1]{}
		\newcommand{\replace}[2]{#2} \newcommand{\replacechunk}[2]{#2}
		\newcommand{\ER}[2]{#1}%\def\red#1{#1}
		\newcommand{\marginER}[2][0]{}
		\newcommand{\inlineER}[1]{}
		\newcommand{\ERreplace}[3]{#2}
		\newcommand{\rmk}[2]{} 
		\newcommand{\draftfootnote}[1]{}\def\crosstwo{}\def\crossone{}\def\gray#1{}

	% I still use refcheck in two-cols mode. Comment this line not to.
	%    \usepackage{refcheck}  \textwidth 44pc \columnsep 2pc  \addtolength{\oddsidemargin}{-0in}
\fi

%-----all these are only for the draft version -----^
%% %---- Drafts ----^
